Cryogenic operation of MEMS-based suspended high overtone bulk acoustic wave resonators for microwave to optical signal transduction

Suspended high-overtone bulk acoustic wave resonators (HBARs) can serve as a viable optomechanical platform for efficient transduction of signals from the microwave to the optical frequency domain. In contrast to 1D nanobeam optomechanical crystals, HBARs benefit from very high RF to phonon injection efficiency ($\eta_{PIE}\approx$1) and low optical pump induced heating at cryogenic temperatures. By building small mode volume optical cavities around these devices, one can in principle achieve optomechanical cooperativities comparable to 1D nanobeam optomechanical crystals. In this work, we demonstrate cryogenic operation ($\approx$10 K) of such suspended HBAR devices and show classical signal modulation upto 3.5 GHz and response times $\approx$ 524 ns (for the fundamental mode at 340 MHz). While the transduction efficiency is currently limited by the material and device fabrication processes used in this work, we show that with reasonable modifications, efficient quantum transduction is within reach using this approach.

==> Thingstodo.tex <==
Figure 1:

Try and reduce the size and see how it looks
(a) needs a scale bar
(c) needs a scale bar
the inset cross-section needs to be flipped

Figure 2:

increase the font size for the x and y axis for both the figures
I like to make the boundary of the plots bold, see if that helps
Make the plot in Fig.(a) dark blue so that it prints better

(b) y-label should be Qm rather than Q
Add the Q of the 340 MHz modes as well here

Figure 3:

Add the (a,b,c) labels to the figures
for (c), the font sizes are too small and the font is differnt from the ones used in the other figures
Remove the labels for the fit lines in the legend (it looks too busy now).

Check the pdf generation again, there seems to be a weird mark at the bottom, you can see it if you zoom in closely

Figure 4:

Curve's linewidths need to be increased (by 0.5-1 point)
Fontsizes should be increased as well, check that the font is the same as used in other figures
dB is italicized in the bottom figure, remove that and also check for consistency overall

The tick marks don't seem to appear on this figure (both top and bottom), check that

Figure 5:

Remove figure (b), we will move that to the appendix. Instead move Fig. 6(a) here, we talk about the AOM array in this section. Also, use the other image (the one where we had 4 independent modulators wired for the scattering matrix measurement instead).

Fig. (a) move this to (b) and change the color of the wires and the bounding boxes (black for wires, dark blue / red for the bounding boxes)

Also check the fonts, make sure it is the same font across all the figures

(c) remove the legends for the fits we will indicate that in the caption, else it looks a but busy

Again, try and increase the fontsize a bit more I usually do set(gca,'FontSize',40). See if that works for you.

Figure 6:

Remove the (a)

(b): text font sizes need to be increased and I need to increase the layer outlines a bit more



